Cross-client Label Propagation for Transductive and Semi-Supervised Federated Learning

We present Cross-Client Label Propagation(XCLP), a new method for transductive federated learning. XCLP estimates a data graph jointly from the data of multiple clients and computes labels for the unlabeled data by propagating label information across the graph. To avoid clients having to share their data with anyone, XCLP employs two cryptographically secure protocols: secure Hamming distance computation and secure summation. We demonstrate two distinct applications of XCLP within federated learning. In the first, we use it in a one-shot way to predict labels for unseen test points. In the second, we use it to repeatedly pseudo-label unlabeled training data in a federated semi-supervised setting. Experiments on both real federated and standard benchmark datasets show that in both applications XCLP achieves higher classification accuracy than alternative approaches.

==> algoLP.tex <==
\SetNlSty{}{}{}
\IncMargin{1.5em}
\begin{algorithm*}[t]
\caption{\texttt{LabelPropagation}}\label{alg:LP}
\Indm  
\Input{data matrix $V$, matrix of partial labels $Y$}
\Indp
$A \gets \text{matrix of pairwise cosine similarities }\;
A_{ij}=\frac{\langle v_i, v_j\rangle}{\|v_i\|\|v_j\|}$   \label{LPline:similarity}\;
$B \gets \text{sparsify} A$ to $k$-NN graph by  
$B_{ij} = \begin{cases}A_{ij} &\text{ if } A_{ij} \in \texttt{top}_{k+1}\big( (A_{is})_{s\in [n]}\big) \text{ and } i\neq j,\\ 0\quad&\text{otherwise}\end{cases}$\label{LPline:sparsify}\;
$W \gets B + B^\trans$\label{LPline:symmetrize}\;
 $\mathcal{W} \gets D^{-\frac{1}{2}}W D^{-\frac{1}{2}}$ \text{ for } $D = \text{diag}(W\textbf{1}_n)$ \label{LPline:normaliseW}\;
 $Z \gets (\text{Id}_n - \alpha \mathcal{W})^{-1}Y$  \label{LPline:solve}\;
$\hat{Z} \gets \text{normalize $Z$ via } \hat{Z}_{ij} = Z_{ij}/(\sum_{c=1}^C Z_{ic})$\label{LPline:normalizeZ}\;
$\hat{y} \gets \text{compute labels via } \hat{y}_i = \argmax_{c\in [C]} \hat{Z}_{ic}$ \label{LPline:labels}\; $\omega \gets \text{compute weights via } \omega_i = 1 - H(\hat{Z}_i)/\log C$
\text{ with $H(p)=-\sum_{j\in[C]}p_j\log p_j$.} \label{LPline:entropy}\;
\Indm  
\Output{labels $\hat{y}$, weights $\omega$}
\Indp
\end{algorithm*}


==> attic.tex <==
\iffalse
\newcommand{\mpm}{\!\pm\!}
\begin{table*}[t]
\centering
\caption{\method for semi-supervised learning: classification accuracy [in \%] on federated CIFAR-10. $m$ is the number of clients, $m_L$ the number of clients with labeled data, $n_L$ is the total number of labels across all clients.
%
\iid and non-\iid refer to how the data is split among the clients. For details, see the main text and~\Cref{app:experiments2}.
}
\label{tab:cifar10-results}
\small\setlength{\tabcolsep}{1pt}
\begin{tabular}{ |c|c|c|c|c|c|c|c|c| }
\hline
\multicolumn{5}{|c|}{\textbf{CIFAR-10, \iid} ($m=100$)} 
&\multicolumn{4}{|c|}{\textbf{CIFAR-10, non-\iid} ($m=100$)} \\
\hline
 & \multicolumn{2}{c|}{$m_L=100$} & \multicolumn{2}{c|}{$m_L=50$} 
 & \multicolumn{2}{c|}{$m_L=100$} & \multicolumn{2}{c|}{$m_L=50$}  \\
 \hline
 \textbf{Method} & $n_L=1000$ & $n_L=5000$ & $n_L=1000$ & $n_L=5000$
 & $n_L=1000$ & $n_L=5000$ & $n_L=1000$ & $n_L=5000$\\
 \hline
 FedAvg (labeled only) & $55.46 \mpm 0.43$& $76.13 \mpm 0.46$& $56.97 \mpm 0.59$ & $80.36 \mpm 0.07$ &             $50.94 \mpm 0.14$& $75.34 \mpm 1.38$& $53.26 \mpm 0.69$ & $79.65\mpm 0.12$ \\\hline
 FedAvg+perclientLP &$61.75\mpm 2.22$ & $85.11 \mpm 0.73$ & $65.29 \mpm 2.50$ & $84.41 \mpm 0.25$ &                $50.94 \mpm 0.14$ & $76.61\mpm 1.50$ & $53.26 \mpm 0.69$ & $79.65\mpm 0.12$ \\
 FedAvg+network & $60.12 \mpm 0.15$ & $79.45\mpm0.31$& $59.14\mpm 0.35$ & $81.04\mpm0.20$ &                        $60.60\mpm0.60$ & $80.07\mpm 0.53$ & $59.82\mpm1.05$ & $81.14\mpm0.23$
 \\
 FedMatch & $50.93\mpm 0.56$ & $72.22\mpm0.14$& $57.10\mpm0.46$ & $77.80\mpm0.32$  &                               $50.71\mpm1.57$ & $71.99\mpm0.70$ & $48.24\mpm0.86$ & $66.37\mpm 0.41$ \\
 FedSiam & $67.02\mpm0.98$ & $82.06\mpm0.56 $& $62.98\mpm1.61$ & $78.45\mpm0.34$  &                                $67.85\mpm 0.26$ & $82.23\mpm0.46$& $62.29\mpm1.84$ & $78.84\mpm0.72$  \\
 FedSem+ & $59.98\mpm 0.49$ & $79.49\mpm0.15$& $59.67\mpm 0.47$& $80.94\mpm 0.25$ &                                $60.93\mpm0.97$ & $79.70 \mpm 0.78$& $59.74\mpm 0.74$ & $81.30 \mpm0.09$ \\
 \Fedprop (ours) & $\bf 70.91\mpm0.71$ & $\bf 86.65 \mpm 0.16$ & $\bf 70.81\mpm 1.65$ & $\bf 86.29\mpm 0.34$ &     $\bf73.76\mpm0.71$ & $\bf 85.53\mpm 0.56$ & $\bf70.0\mpm 1.3$ & $\bf 85.4\mpm 0.4$ \\\hline
 \end{tabular}
\end{table*}
\fi



\subsection{Alternative \texttt{\bfseries SecureHamming} protocol}\label{app:crypto2}

The SHADE protocol discussed in Section~\ref{subsec:crypto} is 
lightweight and flexible due to it reliance on only the oblivious 
transfer primitive. However, it has suboptimal communication cost 
because each Hamming distance is treated independently.
%
In this section, we discuss an alternative method based on 
\emph{fully homomorphic encryption (FHE)} (technically, \emph{somewhat homomorphic
encryption (SWHE)} also suffices)~\cite{acar2018survey}.

FHE is a technique that allows computing functions on encrypted arguments. 
The outcome is an encryption of the value that would have been the result 
of evaluating the target function on the plaintext arguments, but the 
computational devices gain no information about the actual plaintext. 

We exploit this paradigm to compute the Hamming distances of a binary 
vector from clients $i$ with all binary vectors from a client $j$ in 
the following way: 

1) Client $i$ encrypts its own data vector $b^{(i)}\in\{0,1\}^L$, 
using its own public key and transfers the resulting vector 
$\boxed{y}=\boxed{b^{(i)}}$ (boxes indicate encryption)
to client $j$.
%
Because the data is encrypted, client $j$ can extract no 
information about client $i$'s data from this.

2) Client $j$ prepares each of its data vectors, $b^{(j)}\in\{0,1\}^L$, 
as in Section~\ref{subsec:crypto} by adding uniform random values, 
$r_1,\dots,r_L\in[0,L-1]$ to each entry, as well as to the complement 
of each value. 
%
It then encrypts this data with clients $i$'s public key, 
resulting in vectors $\boxed{x}=\boxed{r^{(j)}+b^{(j)}}$, 
and $\boxed{x'}=\boxed{r^{(j)}+(1-b^{(j)})}$.

3) Client $j$ then evaluates the function $f(x,x',y) = 
 \sum_{l=1}^L x_ly_l + x'_l(1-y_l)$ in a fully homomorphic 
 way with arguments $(\boxed{x}, \boxed{x'}, \boxed{y})$.
%
By the same reasoning as in Section~\ref{subsec:crypto}, 
the result is $\boxed{T}=\boxed{\sum\nolimits_l r_l + H(b,b')}$.

4) Client $i$ sends $\boxed{T}$ to client $j$, who decrypts it 
using its own secret key and sends the resulting value $T$ to 
the server. 
%
Client $j$ send the value $R=\sum_l r_l$ to the server. 

5) The server recovers $H(b,b')=T-R$ without gaining other
additional information about the clients' data. 
%
Similarly, client $j$ learns nothing about client $i$'s data
or the Hamming distance value, because of the uniformly 
random shift in the value $T$. 

%\subsubsection{Or?}
%$$h(b,b') = \sum_l(b_lb'_l + (1-b_l)(1-b'_l)) = \sum_{l:b_l=1} b'_l + \sum_{l:b_l=0}(1-b'_l) = n - \sum_l b_l + \sum_{l:b_l=1} b'_l - \sum_{l:b_l=0}b'_l$$

\begin{figure*}[t]
\centering
\subfloat[\emph{Label propagation}. Left: a dataset with 2 labeled data points per class (colored) and many unlabeled ones (black). Right: soft labels for the unlabeled data points are estimated by propagating label information along a 10-nearest-neighbor graph.\label{subfig:LP}]{\includegraphics[width=.28\textwidth,height=.2\textwidth]{images/LP-moons-crop}\includegraphics[width=.28\textwidth,height=.2\textwidth]{images/LP-moons-result-crop}}
\quad
\subfloat[\emph{Locality sensitive hashing}. The expected number of random hyperplanes that separate two data points (here: 2 out of 10) is proportional to the angle between the points.\label{subfig:LSH}]{\qquad\includegraphics[width=.28\textwidth,height=.2\textwidth]{images/LSH-hyperplanes-crop}\qquad}
\caption{Illustration of \emph{label propagation} \protect\subref{subfig:LP} and \emph{locality sensitive hashing}~ \protect\subref{subfig:LSH}.}
\label{fig:background}
\end{figure*}

\input{algoLP}

\myparagraph{Efficiency -- Computational}\quad \method's most costly computation 
steps are multiple matrix multiplications and one matrix inversion operation. 
Overall, however, the computational cost is small compared to the cost of 
training the deep network on the clients. That is because the matrices it 
makes use of scale with the number of data points of the active clients, 
rather than the (typically much larger) number of network parameters. 
%
The same holds for \texttt{CrossClientLP}, which---with the exception 
of the additional LSH steps---performs the same 
computational steps as ordinary LP. 
%
Furthermore, the most expensive steps 
of normalization and matrix inversion are carried out by the server. 
LSH itself requires only one additional
matrix multiplication per client which adds negligible overhead on top of the computation
of client features.
%
By design all cryptographic primitives are chosen to allow maximal efficiency. 
%
For the \texttt{SecureHamming} step,  special-purpose routines, such as SHADE~\citep{bringer2013shade}, rely on \emph{oblivious transfer (OT)}~\citep{ishai2003extending,roy2022softspokenot} as the only cryptographic primitive. Highly optimized libraries exist for this, such as libOTe~\citep{libOTe}, which allows for hundreds of thousands of OT operations per second.  
%
\texttt{SecureSum} can be implemented efficiently using, \eg, 
\emph{secret sharing}~\citep{shamir1979share} or 
\emph{garbled circuits}~\citep{yao1986generate}.
%
A similar secure summation step is already used in FL to 
avoid information leakage during model averaging~\citep{BonawitzIKMMPRS17}.  % overview of MPC: evans2018pragmatic
%
A number of libraries exist that are tailored to this 
task, for instance SAFELearn~\citep{FereidooniMMMMN21},
which allows for aggregation of tens of megabytes per second.
%
%functional secret sharing with Francis Bach: \cite{ryffel2020ariann}
The computational overhead added by both of these methods 
is typically small compared to the training of the network itself.



In a federated setting, running LP jointly on the data of all client is not possible, because, 1) computing the similarity between two data points requires transferring them to a shared 
location, and 2) the propagating step requires labels information to be shared amongst the clients. 

\textcolor{green}{WE NEED TO DISCUSS "MORE DATA GOOD" SOMEWHERE. 
Instead, one could assign labels by running label 
propagation independently on each device, making use of just the 
locally available label.} %\footnote{This is one of our baselines in the experiments.}
%
However, this has a number of drawbacks: first, it can be 
expected lead to lower accuracy in the predicted labels 
compared to label propagation run over all data, because 
computing neighborhood graphs from smaller amounts of 
data makes them less reliable. 
%
Second, the procedure is not applicable at all for clients with 
only unlabeled data.

If not for the constraint of data privacy, classical \textit{label propagation} (LP)~\cite{} would be applicable, which works as follows.
%. For a data matrix $X\in\R^{n\times d}$ with partial labels $Y\in\{-1,0,1\}^n$, it works as follows. 
%
%First, from the set of all pairwise data imilarities, $W=X^\top X$,
First, it builds a neighborhood graph of all available data (labeled and unlabeled) in which pairs of similar points are connected by edges. % weighted?
%
Then, the label information of each labeled data point is propagated to its neighbors in the graph, from which it is propagated to the neighbors' neighbors, \etc.
%
With suitable normalization, this procedure converges, thereby yielding a label estimate for each data point. 
%
\textcolor{blue}{LP starts by computing a matrix of \emph{pairwise similarities} between all data points, which it converts into the adjacency matrix of a graph with weighted edges. 
%
By some algebraic transformations, it 
obtains a matrix that encodes how close 
any data point is to any other point 
with respect to paths in the graph structure. 
%
From the product of this \emph{influence matrix} with the partial label matrix one obtained label predictions for each data point. }
%and a derivation of these steps
For further details, see Appendix~\ref{app:LP}.







Client steps are also unproblematic from a privacy viewpoint, so
what remains is how to execute the cross steps efficiently
yet without sharing client data. 
%
To do so, we transform the problem into a form
that is equivalent but allows for the application 
of tailored cryptographic tools that are 
highly efficient yet fully secure.
%
%
\Cref{alg:crossclientLP} shows pseudo-code for \texttt{CrossClientLP}.
%
For simplicity of exposition, we describe it as if communication between clients were possible, which is a reasonable assumption in a \emph{cross-silo} setting. If this is not possible, as is likely the case in \emph{cross-device} FL, then communication is orchestrated by the server, see \eg \cite{BonawitzIKMMPRS17}.
%




==> crypto.tex <==
% To compute pseudo-labels, we would like to execute 
% label propagation over a 
% cross-client neighborhood graph built from 
% the embedded data of all currently selected clients. 
%
The main difficulty in executing LP across 
multiple clients lies in how to avoid having to
share data among clients without resorting to
highly inefficient tools.
%
By default, \Cref{alg:LP} would require the clients 
to share their $V^{(j)}$ in order to compute inner products 
when forming the similarity matrix $A$ 
(line~\ref{LPline:similarity}) and their $Y^{(j)}$ when 
computing the class score matrix 
$Z$ (line~\ref{LPline:solve}), which would violate the constraints
of a federated setting.
%
A naive solution to overcoming this problem would be to 
execute \Cref{alg:LP} in its entirety using \emph{multi-party 
computation}  (MPC)~\citep{Yao82b,cramer2015secure}, a set of cryptographic tools that---in principle---allow participants to jointly 
compute any function in a way that leaks no information 
to any of them. 
%
However, for complicated functions of real-valued inputs,
such as matrix inversion, MPC has high computational and 
communication overhead and would not be practical. 
%
%
%\textcolor{blue}{For a formal analysis, see Appendix~\ref{app:crypto}.}



==> fedisic-curves.tex <==
\begin{figure*}[t]
\caption{CCLP for prediction (Fed-ISIC2019 dataset): classification accuracy [in \%] 
for \method and baselines for representations obtained with communication rounds and 
when different amounts, $n$, of overall training data.}\label{fig:fedisic_figure} 
\begin{tabular}{cccc}
\includegraphics[width=.23\textwidth]{images/training_curve_frac_0.05}&
\includegraphics[width=.23\textwidth]{images/training_curve_frac_0.1}&
\includegraphics[width=.23\textwidth]{images/training_curve_frac_0.2}&
\includegraphics[width=.23\textwidth]{images/training_curve_frac_1}
\\
$n=1234$ & $n=2346$ & $n=3456$ & $n=4567$
\end{tabular}
\end{figure*}

==> preliminaries.tex <==
\section{Preliminaries}
In this section we first define our notation. Then in \Cref{subsec:LP} we introduce label propagation in the standard (non-federated) setting. 
Finally, in \Cref{subsec:LSH}, we introduce locality-sensitive hashing, a key tool we make use of in \method.

We assume a federated classification setting with $m$ clients coordinated by a central server. Each client $j$ possesses partly labeled data $(X^{(j)}_L, y^{(j)}_L, X^{(j)}_U)$ with $X^{(j)}_L \coloneqq \{x_1^{(j)}, \dots, x_{l^{(j)}}^{(j)}\}$, $y^{(j)}_L\coloneqq \{y_1^{(j)}, \dots, y_{l^{(j)}}^{(j)}\}$ and $X^{(j)}_U\coloneqq \{x_{l^{(j)}+1}^{(j)}, \dots, x_{n^{(j)}}^{(j)}\}$. Here $l^{(j)}$ and $n^{(j)}$ denote the number of labels and the total number of data points owned by client $j$. We state the problem in this way to be fully general, note that in some settings a client may have only labeled data, $n^{(j)} = l^{(j)}$ or only unlabeled data, $l^{(j)} = 0$. Let $D$ denote the data dimension, so that $x_i^{(j)} \in \R^D$, and $C$ the number of classes, so that $y_i^{(j)} \in [C] \coloneqq\{1, \dots, C\}$. 
%
We further denote by $f_\theta : \mathbb{R}^D \rightarrow \mathbb{R}^C$ a parametric classifier of the data, with parameters $\theta$, which in our case is a deep neural network. We decompose $f_\theta$ into a feature extractor $f_\phi : \mathbb{R}^D \rightarrow \mathbb{R}^{d}$ and a classifier head $f_\psi : \mathbb{R}^{d} \rightarrow \mathbb{R}^C$, so that $f_\theta = f_\psi \circ f_\phi$ with $\theta=(\psi,\phi)$. In standard fashion, $f_\theta$ will be trained by stochastic gradient optimization of a loss function 
%
$L(X, Y, \omega ; \theta) = \sum_{i=1}^n \omega_i \ell(f_\theta(x_i), y_i)$, where 
$\omega_i$ are per-sample weights and $\ell$ is the cross entropy loss.

\subsection{Label Propagation (LP)} \label{subsec:LP}
Given partly labeled data, LP is a classic 
technique for directly assigning labels to the unlabeled data. We describe a variant of the graph-based diffusion approach of \cite{label_prop}. 
%
The key idea is to propagate label information from labeled to unlabeled points 
taking into account the geometry of the underlying data manifold, see \Cref{subfig:LP} for an illustration.
%
The manifold is approximated by a neighborhood graph of the data, in which points are connected based on how similar they are. 

\Cref{alg:LP} describes the procedure in pseudocode.
%
As input, it takes a set of data vectors, $V = V_L \cup V_U = \{v_1, \dots v_{l}, v_{l + 1}, \dots v_{n}\}$,
and partial labels $\{y_1,\dots,y_{l}\}$ from $C$ classes, which we encode in one-hot matrix form: 
$Y\in\R^{n\times C}$ with $Y_{ic} = \mathbbm{1}_{(y_i = c)}$ for $i\leq l$ and $Y_{ic}=0$ otherwise.
%
The algorithm starts by computing a matrix $A\in\R^{n\times n}$ of pairwise 
similarities between all data points (line \ref{LPline:similarity}).
%
$A$ is sparsified by keeping only each point's $k$ nearest 
neighbors, symmetrized, and then normalized (lines \ref{LPline:sparsify}--\ref{LPline:normaliseW}), resulting in a transition matrix, $\mathcal{W}$.
%
Label propagation now amounts to repeatedly spreading label information 
across the resulting graph by multiplying with $\alpha \mathcal{W}$ until convergence, 
where $\alpha \in (0,1)$ is a hyper-parameter reflecting how much the 
algorithm should weight the original labels. 
%
The outcome of this can be computed in closed form (line \ref{LPline:solve}).
The resulting matrix, $Z \in \mathbb{R}^{n \times C}$, 
can be interpreted as unnormalized class scores for each data point. 
%
Normalizing $Z$ across rows 
yields, for each point, a probability distribution across all classes (line \ref{LPline:normalizeZ}). 
%
From this, one assigns a maximum-likelihood label to each point (line \ref{LPline:labels})
as well as a weight reflecting the confidence in the assignment based on 
the entropy of class probabilities (line \ref{LPline:entropy}).

\subsection{Locality-Sensitive Hashing (LSH)} \label{subsec:LSH}
LSH~\citep{indyk1998approximate} is a procedure for hashing real-valued vectors into binary vectors
while preserving their similarity. Let $v\in\R^d$ be a vector. To encode $v$ into a binary vector $b$ of length $L$, LSH randomly samples $L$ hyperplanes in $\R^d$. For each hyperplane it checks whether $v$ lies above or below it and sets the $i$th bit in $b$ as $1$ or $0$ accordingly.
%
Formally, $b_i = \mathbbm{1}_{\langle v, u_i \rangle\geq 0}$, where 
$u_i \in \R^d$ is the normal vector of the $i$th hyperplane. 
%
A key property of LSH is that it approximately preserves cosine-similarity.
%that from the bit-vector encoding, one can approximately recover the cosine similarity. it (in expectation) preserves . 
Concretely, for vectors $v_1,v_2$ with LSH encodings $b_1, b_2$, one has 
%
$%\begin{equation}\label{eq:hamming_cosine}
    \frac{\langle v_1, v_2\rangle}{\|v_1\|\|v_2\|} \approx \cos( \pi H(b_1, b_2)/L)$
    %\end{equation}
where $H$ is the Hamming distance (number of bits that differ) between two binary vectors. 
%
The reason is that the probability of $b_1$ and $b_2$ differing at 
any bit $i$ is the probability that the $i$th sampled hyperplane 
lies between $v_1$ and $v_2$, which is equal to $\angle(v_1,v_2)/\pi$, 
see \Cref{subfig:LSH}. % for an illustration.
%
By the law of large numbers, the more hyperplanes one samples, the better the approximation quality. 
%sample a random hyperplane and for each point record as $s_i$ and $s_j$ on which side of the hyperplane the points fall.
%%
%Consequently, the expected value of the indicator $\textbf{1}_{[(b_1)_i\neq(b_2)_i]}$ is $\frac{\angle(v_1,v_2)}{\pi}$ and the empirical estimate of this expectation is exactly $\frac{H(b_1, b_2)}{L}$. Rearranging and taking the cosine of both sides leads to \cref{eq:hamming_cosine}. 

\input{algoLP.tex}


==> tables/cifar10.tex <==
\begin{table}[t]
\caption{caption}
\label{tab:cifar10-results}
\begin{center}
\tiny
% \begin{center}
\begin{tabular}{ |c|c|c|c|c|c|c| }
\hline
\multicolumn{7}{|c|}{\textbf{CIFAR-10, IID}} \\
\hline
 & \multicolumn{2}{c|}{\textit{Labels-At-Client} ($m_L=100$)} & \multicolumn{2}{c|}{\textit{Labels-At-Client} ($m_L=50$)} & \multicolumn{2}{c|}{\textit{Labels-At-Server}} \\
 \hline
 \textbf{Method} & 1000 labels & 5000 labels & 1000 labels & 5000 labels & 1000 labels & 5000 labels\\
 \hline
 FedAvg (Supervised) & $55.46 \pm 0.43 \%$& $76.13 \pm 0.46 \%$& $56.97 \pm 0.59 \%$ & $80.36 \pm 0.07 \%$ &$62.06 \pm 0.38 \%$  & $81.96 \pm 0.32 \%$ \\
 FedAvg + local LP & & & & & & \\
 FedAvg + MT & & $84.92 \pm 0.64\%$ & & & & \\
 \hline
 FedMatch & $49.50 \pm 0.22 \%$ & $72.52 \pm 0.78\%$& && & \\
 FedSiam & $69.58 \pm 0.06 \%$ & $83.62 \pm 0.26 \%$& & & - & 80.50 \\
 FedLP &$59.63 \pm 1.01 \%$ & $86.50 \pm 0.34 \%$ & $59.85 \pm 1.11$ & $79.39 \pm 0.14 \%$ & $70.21 \pm 0.35 \%$ & $84.46 \pm 0.45 \%$ \\
 \hline
 \multicolumn{7}{|c|}{\textbf{CIFAR-10, NONIID}} \\
\hline
 & \multicolumn{2}{c|}{\textit{Labels-At-Client} ($m_L=100$)} & \multicolumn{2}{c|}{\textit{Labels-At-Client} ($m_L=50$)} & \multicolumn{2}{c|}{\textit{Labels-At-Server}} \\
 \hline
 \textbf{Method} & 1000 labels & 5000 labels & 1000 labels & 5000 labels & 1000 labels & 5000 labels\\
 \hline
 FedAvg (Supervised) & $47.47 \pm 1.16$& $70.35 \pm 0.60$& $50.32 \pm 0.16$ & $72.29 \pm 0.03$ &$55.81 \pm 1.16$  & $76.42 \pm 0.24$ \\
 FedAvg + local LP & & $61.76$ & & & & \\
 \hline
 FedMatch & & & && & \\
 FedSiam & - & & & & - & \\
 FedLP & & & & & & \\
 \hline
\end{tabular}
\end{center}
\end{table}

% \begin{table}[t]
% \caption{Sample table title}
% \label{sample-table}
% \begin{center}
% \begin{tabular}{ll}
% \multicolumn{1}{c}{\bf PART}  &\multicolumn{1}{c}{\bf DESCRIPTION}
% \\ \hline \\
% Dendrite         &Input terminal \\
% Axon             &Output terminal \\
% Soma             &Cell body (contains cell nucleus) \\
% \end{tabular}
% \end{center}
% \end{table}

==> tables/cifar100.tex <==


\begin{table}[t]
\caption{}
\label{tab:cifar100-results}
\begin{center}
\small
% \begin{center}
\begin{tabular}{ |c|c|c| }
\hline
\multicolumn{3}{|c|}{\textbf{CIFAR-100, IID}} \\
\hline
 & $m=m_L=50$  & $m=m_L=100$ \\
 \hline
 \textbf{Method} & $N_L = 5000$ & $N_L=10000$ \\
 \hline
 FedAvg (Supervised) & $43.80 \pm 0.19 $& $53.91 \pm 0.25 $ \\
 FedAvg + local LP & $43.82 \pm 0.59 $ & $54.38 \pm 0.36 $ \\
 FedAvg + MT & $49.09 \pm 0.38$ & $56.05\pm 0.23$ \\
 \hline
 \Fedprop & $50.19\pm 0.60$ & $57.00 \pm 0.08$ \\
 \Fedprop + MT &$50.60 \pm0.28$& $58.66\pm 0.28$  \\
 \hline
\end{tabular}
\end{center}
\end{table}


% \begin{table}[t]
% \caption{}
% \label{cifar100-results}
% \begin{center}
% \small
% % \begin{center}
% \begin{tabular}{ |c|c|c| }
% \hline
% \multicolumn{3}{|c|}{\textbf{CIFAR-100, IID}} \\
% \hline
%  & \multicolumn{2}{c|}{\textit{Labels-At-Client}} \\
%  \hline
%  \textbf{Method} & 5000 labels & 10000 labels\\
%  \hline
%  FedAvg (Supervised) & $43.80 \pm 0.19 \%$& $53.91 \pm 0.25 \%$ \\
%  FedAvg + local LP & $43.82 \pm 0.59 \%$ & $54.38 \pm 0.36 \%$ \\
%  FedAvg + MT & $49.09 \pm 0.38 \%$ & $53.45 \pm 0.16 \%$ \\
%  \hline
%  \method & $48.31 \pm 0.50 \%$ & $56.29 \pm 0.16 \%$ \\
%  \hline
% \end{tabular}
% \end{center}
% \end{table}

==> tables/fedisic.tex <==
% \begin{table*}[t]
% \caption{\method for prediction: Classification accuracy [in \%] when different fractions, $\alpha$, of training data are labeled. {FedAvg} and \emph{\method(labeled)} use only the labeled part of the training set, \emph{\method(full)} uses also the unlabeled part (Fed-ISIC2019 dataset).}
% \label{tab:fedisic_results}
% \begin{center}
% \small
% % \begin{center}
% \begin{tabular}{ |c|c|c|c|c|c|c|c| }
% \hline
%  & $\alpha=0.05$ & $\alpha=0.1$ & $\alpha=0.2$ & $\alpha=0.4$ & $\alpha=0.6$ & $\alpha=0.8$ & $\alpha=1.0$ \\
%  \hline
% %\method (pretrained features) & 34.65 & 37.93 & 40.17 & 45.86 & 47.81 & 50.77 & 53.24 \\
% %\method (pretrained features, no unlabeled training data) & 33.64 & 34.27 & 38.20 & 44.76 & 46.84 & 50.52 & 53.24 \\
% \emph{FedAvg}  & $43.78 \pm 0.88$ & $46.83 \pm 0.75$ & $52.87 \pm 0.14$ & $57.67 \pm 0.72$ & $60.53 \pm 1.79$ & $62.89 \pm 1.24$ & $63.78 \pm 0.20$ \\
% \emph{\method(labeled)} & $47.48 \pm 1.12$ & $50.95 \pm 1.80$ & $58.08 \pm 0.60$ & $63.84 \pm 0.79$ & $67.70 \pm 1.08$ & $70.18 \pm 0.12$ & $73.31 \pm 0.67$ \\
% \emph{\method(full)}& $48.89 \pm 1.54$ & $52.92 \pm 0.93$ & $61.09 \pm 0.66$ & $66.10 \pm 1.03$ & $69.34 \pm 0.32$ & $71.53 \pm 0.35$ & $73.31 \pm 0.67$ \\
%  \hline
% \end{tabular}
% \end{center}
% \end{table*}

% \begin{table}[t]
% \caption{\method for prediction: Classification accuracy [in \%] when different fractions, $\alpha$, of training data are labeled. {FedAvg} and \emph{\method(labeled)} use only the labeled part of the training set, \emph{\method(full)} uses also the unlabeled part (Fed-ISIC2019 dataset).}
% \label{tab:fedisic_results}
% \begin{center}
% \small
% % \begin{center}
% \begin{tabular}{ |c|c|c|c|c|c|c|c| }
% \hline
%  & $\alpha=0.05$ & $\alpha=0.1$ & $\alpha=0.2$ & $\alpha=1.0$ \\
%  \hline
% %\method (pretrained features) & 34.65 & 37.93 & 40.17 & 45.86 & 47.81 & 50.77 & 53.24 \\
% %\method (pretrained features, no unlabeled training data) & 33.64 & 34.27 & 38.20 & 44.76 & 46.84 & 50.52 & 53.24 \\
% \emph{FedAvg}  & $43.78 \pm 0.88$ & $46.83 \pm 0.75$ & $52.87 \pm 0.14$ & $63.78 \pm 0.20$ \\
% \emph{\method(labeled)} & $47.48 \pm 1.12$ & $52.34 \pm 0.93$ & $59.49 \pm 0.88$ & $74.22 \pm 0.67$ \\
% \emph{\method(full)}& $49.50 \pm 1.42$ & $53.78 \pm 0.90$ & $61.09 \pm 0.66$ &  $74.22 \pm 0.67$ \\
%  \hline
% \end{tabular}
% \end{center}
% \end{table}


==> tables/miniimagenet.tex <==
\begin{table}[t]
\caption{}
\label{tab:miniimagenet-results}
\begin{center}
\small
% \begin{center}
\begin{tabular}{ |c|c|c| }
\hline
\multicolumn{3}{|c|}{\textbf{Mini-Imagenet, IID}} \\
\hline
 & \multicolumn{2}{c|}{\textit{Labels-At-Client}} \\
 \hline
 \textbf{Method} & 5000 labels & 10000 labels\\
 \hline
 FedAvg (Supervised) & $23.39 \pm 0.52$& $31.72 \pm 0.54 $ \\
 FedAvg + local LP & $25.53\pm 0.22$ & $33.09\pm 0.62$ \\
 FedAvg + MT & $25.98\pm 0.70$ & $33.20\pm 0.68$ \\
 \hline
 \method & $26.93\pm 0.41 $ & $35.78\pm 0.56 $ \\
 \method + MT & & $33.24\pm 0.71$  \\
 \hline
\end{tabular}
\end{center}
\end{table}

% \begin{table}
% \caption{}
% \label{miniimagenet-results}
% \begin{center}
% \tiny
% % \begin{center}
% \begin{tabular}{ |c|c|c|c|c| }
% \hline
% \multicolumn{5}{|c|}{\textbf{Mini-Imagenet, IID}} \\
% \hline
%  & \multicolumn{2}{c|}{\textit{Labels-At-Client}} & \multicolumn{2}{c|}{\textit{Labels-At-Server}} \\
%  \hline
%  \textbf{Method} & 5000 labels & 10000 labels & 5000 labels & 10000 labels\\
%  \hline
%  FedAvg (Supervised) & $23.39 \pm 0.52 \%$& $31.72 \pm 0.54 \%$ &  &  \\
%  FedAvg + local LP & & & & \\
%  \hline
%  \method & $26.21 \pm 0.26 \%$ & $35.79 \pm 0.60 \%$ & & \\
%  \hline
% \end{tabular}
% \end{center}
% \end{table}
